Distributed Certifiably Correct Pose-Graph Optimization

This paper presents the first certifiably correct algorithm for distributed pose-graph optimization (PGO), the backbone of modern collaborative simultaneous localization and mapping (CSLAM) and camera network localization (CNL) systems. Our method is based upon a sparse semidefinite relaxation that we prove provides globally-optimal PGO solutions under moderate measurement noise (matching the guarantees enjoyed by state-of-the-art centralized methods), but is amenable to distributed optimization using the low-rank Riemannian Staircase framework. To implement the Riemannian Staircase in the distributed setting, we develop Riemannian block coordinate descent (RBCD), a novel method for (locally) minimizing a function over a product of Riemannian manifolds. We also propose the first distributed solution verification and saddle escape methods to certify the global optimality of critical points recovered via RBCD, and to descend from suboptimal critical points (if necessary). All components of our approach are inherently decentralized: they require only local communication, provide privacy protection, and are easily parallelizable. Extensive evaluations on synthetic and real-world datasets demonstrate that the proposed method correctly recovers globally optimal solutions under moderate noise, and outperforms alternative distributed techniques in terms of solution precision and convergence speed.

==> convergence.tex <==
\section{Convergence Analysis for Riemannian Block-Coordinate Descent}
\label{sec:convergence}


In this section, we formally establish first-order convergence guarantees for RBCD (Algorithm~\ref{alg:BCD}) and its accelerated variant $\ARBCD$ (Algorithm~\ref{alg:ARBCD}).
We first focus on the rank-restricted semidefinite relaxation of PGO (Problem~\ref{prob:se_sync_riemannian}) and prove convergence of $\RBCD$ and $\ARBCD$ on this problem.
Later in this section, we remark on how our guarantee directly generalizes to a much broader setting (e.g., with general smooth cost functions).
We begin with the following lemma, which states that the Riemannian gradients of the reduced problem of Problem~\ref{prob:se_sync_riemannian} satisfy a Lipschitz-type condition.


\begin{lemma}[Lipschitz-type gradient for pullbacks]
	In Problem~\ref{prob:se_sync_riemannian}, consider the reduced cost $f_b$ and its pullback $\fhat_b$ for an arbitrary block $b \in [N]$.
	There exists a constant $c_b \geq 0$ such that for any $X_b \in \Mcal_b$ and $\eta_b \in T_{X_b} \Mcal_b$,
	\begin{equation}
	\big|\fhat_b(\eta_b) - [f_b(X_b) + \langle \eta_b, \rgrad f_b(X_b) \rangle]\big| \leq \frac{c_b}{2} \norm{\eta_b}^2_2.
	\label{eq:lipschitz_gradient_pullback}
	\end{equation}
	\label{lem:lipschitz}
\end{lemma}

In \cite{Boumal2018Convergence}, Boumal et al. use  \eqref{eq:lipschitz_gradient_pullback} as a convenient generalization of the classical property of Lipschitz continuous gradient. 
With this property, the authors show that it is straightforward to establish global first-order convergence guarantees, e.g., for the well-known Riemannian gradient descent algorithm.
In this work, we follow a very similar proof strategy as presented in \cite{Boumal2018Convergence}, and provide global convergence rate estimates for the proposed $\RBCD$ and $\ARBCD$ algorithm.
Our convergence analysis relies on the following very mild assumptions.



\begin{assumption}[Assumptions on Algorithm~\ref{alg:BlockUpdate}]
	When using Algorithm~\ref{alg:BlockUpdate} to update individual blocks, we require the following assumptions to hold.
	\begin{enumerate}
		\item
		The user-specified map $H$ in the model function \eqref{eq:reduced_model} is globally radially linear, i.e.,
		\begin{equation}
		H[c \eta_b] = c H[\eta_b], \, \text{ for all } \eta_b \in T_{X_b} \Mcal_b \text{ and } c \geq 0.
		\end{equation}
		\item Let $X^0, X^1, \hdots, X^K$ denote the iterates of $\RBCD$ or $\ARBCD$. 
		There exists $c_0 \geq 0$ such that for any iteration $k = 0, 1, \hdots$ and block $b \in [N]$, 
		\begin{equation}
		\max_{\eta_b \in T_{X^k_b} \Mcal_b, \norm{\eta_b} \leq 1} |\langle \eta_b, H[\eta_b] \rangle| \leq c_0.
		\label{eq:H_bounded}
		\end{equation}
		\item 
		The initial trust-region radius, denoted as $\Delta_0$, is bounded away from zero by,
		\begin{equation}
		\Delta_0 \geq \lambda_{b} \norm{\rgrad_{X_b} f_b},
		\end{equation}
		where $X_b$ is the input block estimate to Algorithm~\ref{alg:BlockUpdate}
		and $\lambda_b$ is a block-specific constant defined as, 
		\begin{equation}
		\lambda_b \triangleq \frac{1}{8(c_b + c_0)}. 
		\label{eq:lambda_b}
		\end{equation}
	\end{enumerate}
	\label{assumption_rtr}
\end{assumption}

We note that the first two regularity conditions in Assumption~\ref{assumption_rtr} are the same as Assumption A.6 in \cite{Boumal2018Convergence}. 
As discussed by Boumal et al. \cite{Boumal2018Convergence}, these two conditions are fairly lax; in particular, the simplest choice of $H$ that satisfies the requirements is the identity mapping.
In our implementation, we use the Riemannian Hessian at the selected block $\Hess f_b(X_b)$ for faster convergence.\footnote{
	In Appendix~\ref{sec:hessian_discussion}, we provide a rigorous proof that the Riemannian Hessian satisfies the boundedness assumption \eqref{eq:H_bounded} for all of the iterates generated by $\RBCD$ and $\ARBCD$. }
Finally, 
the last condition in Assumption~\ref{assumption_rtr} can be easily satisfied by using a sufficiently large initial trust-region radius. 
Using Lemma~\ref{lem:lipschitz} and Assumption~\ref{assumption_rtr}, we can now prove that each block update (Algorithm~\ref{alg:BlockUpdate}) yields \emph{sufficient descent} on the corresponding reduced cost function.

\begin{lemma}[Sufficient descent property of Algorithm~\ref{alg:BlockUpdate}]
	Under Lemma~\ref{lem:lipschitz} and
	Assumption~\ref{assumption_rtr}, applying \textsc{BlockUpdate} (Algorithm~\ref{alg:BlockUpdate}) on a block $b \in [N]$ with an input value $X_b^k$ decreases the reduced cost by at least,
	\begin{equation}
	f_{b}(X^{k}_{b}) - f_{b}(X^{k+1}_{b}) \geq \frac{1}{4} \lambda_{b} \norm{\rgrad f_{b}(X_{b}^k)}^2,
	\end{equation}
	where $\lambda_{b}$ is the block-specific constant corresponding to the selected block defined in \eqref{eq:lambda_b}.
	\label{lem:sufficient_decrease}
\end{lemma}

Lemma~\ref{lem:sufficient_decrease} states that after each iteration of $\RBCD$, we are guaranteed to decrease the corresponding reduced cost function. 
Furthermore, the amount of reduction is \emph{lower bounded} by some constant times the squared gradient norm at the selected block.  
Thus, if we execute $\RBCD$ for long enough, intuitively we should expect the iterates to converge to a solution where the gradient norm is zero (i.e., a first-order critical point). The following theorem formalizes this result.

\begin{theorem}[Global convergence rate of $\RBCD$]
	Let  $f^\star$ denote the global minimum of the optimization problem
	\eqref{eq:manopt_problem}.
	Denote the iterates of $\RBCD$ (Algorithm~\ref{alg:BCD}) as 
	$X^0, X^1, \hdots, X^{K-1}$, and the corresponding block selected at each iteration as $b_0, \hdots, b_{K-1}$.
	Under Lemma~\ref{lem:lipschitz} and
	Assumption~\ref{assumption_rtr}, $\RBCD$ with \emph{uniform sampling} or \emph{importance sampling}
	have the following guarantees,
	\begin{equation}
	\min_{0 \leq k \leq K-1} \mathbb{E}_{b_{0:k-1}}\norm{\rgrad f(X^k)}^2 \leq \frac{4N (f(X^0) - f^\star)}{K \cdot \min_{b \in [N]}\lambda_b }.
	\label{eq:general_convergence_uniform}
	\end{equation}
	In addition, $\RBCD$ with \emph{greedy selection}
	yields the following \emph{deterministic} guarantee,
	\begin{equation}
	\min_{0 \leq k \leq K-1} \norm{\rgrad f(X^k)}^2 \leq \frac{4N(f(X^0) -
	f^\star)}{K \cdot \min_{b \in [N]}\lambda_b }.
	\label{eq:general_convergence_greedy}
	\end{equation}
	\label{thm:general_convergence}
\end{theorem}

Theorem~\ref{thm:general_convergence} establishes a \emph{global} sublinear convergence rate for $\RBCD$.\footnote{
	We note that in our current analysis, uniform sampling and importance sampling share the same convergence rate estimate. 
	In practice, however, it is usually the case that importance sampling yields much faster empirical convergence (see Section~\ref{sec:experiments}). 
	This result suggests that it is possible to further improve the convergence guarantees for importance sampling. We leave this for future work.}
Specifically, as the number of iterations $K$ increases, the squared gradient norm decreases at the rate of $\mathcal{O}(1/K)$.
Using the same proof technique, we can establish a similar convergence guarantee for the accelerated version $\ARBCD$. 

\begin{theorem}[Global convergence rate of $\ARBCD$]
	Let  $f^\star$ denote the global minimum of the optimization problem
	\eqref{eq:manopt_problem}.
	Denote the iterates of $\ARBCD$ (Algorithm~\ref{alg:ARBCD}) as 
	$X^0, X^1, \hdots, X^{K-1}$, and the corresponding block selected at each iteration as $b_0, \hdots, b_{K-1}$.
	Define the constant, 
	\begin{equation}
		C \triangleq \min\left(c_1, \min_{b \in [N]} \lambda_b/4\right).
	\end{equation}
	Under Lemma~\ref{lem:lipschitz} and Assumption~\ref{assumption_rtr}, $\ARBCD$ with \emph{uniform sampling} or \emph{importance sampling}
	have the following guarantees,
	\begin{equation}
	\min_{0 \leq k \leq K-1} \mathbb{E}_{b_{0:k-1}}\norm{\rgrad f(X^k)}^2 \leq {CN (f(X^0) - f^\star)}/{K}.
	\label{eq:accelerated_convergence_uniform}
	\end{equation}
	In addition, $\ARBCD$ with \emph{greedy selection}
	yields the following \emph{deterministic} guarantee,
	\begin{equation}
	\min_{0 \leq k \leq K-1} \norm{\rgrad f(X^k)}^2 \leq {CN(f(X^0) - f^\star)}/{K}.
	\label{eq:accelerated_convergence_greedy}
	\end{equation}
	\label{thm:accelerated_convergence}
\end{theorem}


We conclude this section with two remarks that illustrate the \emph{generality} of our convergence guarantees, as they directly extend to general cost functions and more complex blocking schemes.

\begin{remark}[Convergence under general cost functions]
	While we focus on Problem~\ref{prob:se_sync_riemannian},
	it is worth noting that the convergence guarantees derived in this section hold on \emph{any} problem defined on product manifold that satisfies the Lipschitz-type condition 
	\eqref{eq:lipschitz_gradient_pullback}.
	Indeed, as we show in detail in Appendix~\ref{apx:convergence_proof}, our proofs of Theorem~\ref{thm:general_convergence} and Theorem~\ref{thm:accelerated_convergence} only require \eqref{eq:lipschitz_gradient_pullback} and Assumption~\ref{assumption_rtr}. 
	Furthermore, as we discuss in Appendix~\ref{apx:convergence_proof}, the Lipschitz-type condition is easily satisfied in practice, e.g., when the extended cost function (i.e., defined on the ambient space) is Lipschitz smooth and the manifold is compact \cite{Boumal2018Convergence}.
	Because of these general facts, we believe that our algorithm and the convergence guarantees are also of interest to the broader optimization community.
\end{remark}



\begin{remark}[Convergence under parallel executions]
	With the parallel iterations described in Section~\ref{sec:parallel_execution}, 
	we can further improve the global convergence rates of RBCD and $\ARBCD$
	in Theorems~\ref{thm:general_convergence} and
	\ref{thm:accelerated_convergence}.
	For example, the constant $N$ that appears in the rate estimates of uniform sampling and importance sampling \eqref{eq:general_convergence_uniform} can be replaced by the number of aggregate blocks (colors) in the dependency graph.
	Recall that in practice, this is typically bounded by a small constant,
	e.g., the maximum degree in the sparse robot-level dependency graph (see
	Section~\ref{sec:parallel_execution}).
	\label{rem:parallel_convergence}
\end{remark}


